Partial Identification of Treatment Effects with Implicit Generative Models

We consider the problem of partial identification, the estimation of bounds on the treatment effects from observational data. Although studied using discrete treatment variables or in specific causal graphs (e.g., instrumental variables), partial identification has been recently explored using tools from deep generative modeling. We propose a new method for partial identification of average treatment effects(ATEs) in general causal graphs using implicit generative models comprising continuous and discrete random variables. Since ATE with continuous treatment is generally non-regular, we leverage the partial derivatives of response functions to define a regular approximation of ATE, a quantity we call uniform average treatment derivative (UATD). We prove that our algorithm converges to tight bounds on ATE in linear structural causal models (SCMs). For nonlinear SCMs, we empirically show that using UATD leads to tighter and more stable bounds than methods that directly optimize the ATE.

==> figures/background.tex <==
In this section, we introduce the definitions and assumptions we will use throughout the paper. Consider the observed data as (possibly continuous) random variables $\vect{V} = \{X_1, \cdots, X_m, T, Y\} \in \R^d$, where $T$, $Y$, and $\{X_1, \cdots, X_m\}$ denote the treatment variable, target variable, and covariates, respectively.

\subsection{Data generating model}
Our approach will be based on the framework of Structural Causal Models (SCMs). An SCM is a tuple $\scm = (\vect{V}, \vect{U}, \Fcal, P_{\vect{U}})$, where each observed variable $V_i \in \vect{V}$ is a deterministic function of a subset of observed variables $\vect{pa}(V_i) \subseteq \vect{V}$ and latent variables $\vect{U}_{V_i} \subseteq \vect{U}$, i.e.,
\begin{align}
    & V_i = f_{V_i}(\vect{pa}(V_i), \vect{U}_{V_i}) \text{ where } f_{V_i} \in \Fcal,\ V_i \not\in \vect{pa}(V_i)
    \label{def:scm}
\end{align}
Note that in this model, the only source of randomness are latent variables $\vect{U}$ with probability space $(\Omega, \Sigma, P_{\vect{U}})$. This induces a probability law over the observed variables $P_{\scm}$. We may omit the subscript $\scm$ and denote the observational probability distribution by $P$ throughout the text.

Given $\scm$, one can construct a graph with nodes $\vect{V} \cup \vect{U}$ and directed edges from nodes in $\vect{pa}(V_i) \cup \vect{U}_{V_i}$ to $V_i$. We call this graph the causal graph corresponding to SCM $\scm$ and denote it by $\graph_\scm$ or simply $\graph$. Note that $\graph$ is acyclic.

\begin{assump}
Random variables $\vect{V}$ are generated based on an unknown SCM $\scm$. We assume the corresponding causal graph $\graph$ is known.
\end{assump}

\subsection{Causal effect and response function}
For any observed random variable $V$ in the SCM $\scm$, let $V_\scm(\vect{u})$ be its deterministic value after fixing a realization $\vect{u}$ of latent variables $\vect{U}$. We define the causal effect of treatment $T$ on target $Y$ as follows:
\begin{definition}[Causal Effect]
Let $Y_{\scm(T=t)}(\vect{u})$ be the value of $Y$ by fixing $\vect{U}=\vect{u}$ and changing the function $f_T$ to a constant function $f_T = t$ in $\scm$. Then, we call the random variable $Y_{\scm(T=t)}$ the causal effect of treatment $T=t$ on target $Y$. We may simplify the notation and write it as $Y_{t}$ if the SCM $\scm$ and treatment variable $T$ are known from context. Note that $Y_{T(\vect{u})}(\vect{u}) = Y(\vect{u})$.
\end{definition}
\vspace{-0.5em}
One can see $\{Y_t: t \in supp(T)\}$ as a stochastic process defined on $(\Omega, \Sigma, P_{\vect{U}})$, which we call the response function. The response function is also known as partial dependence plot, dose-response curve, and response curve in literature [cite].

\subsection{Average treatment derivative and average dose effect}
In this work, our goal is to estimate the effectiveness of a treatment regime on a population from the observational
distribution $P$ and the causal graph $\graph$.
%
In the case of binary treatments, the effectiveness can be estimated using the average treatment effect (ATE), i.e.,
$\E[Y_1] - \E[Y_0]$.
%
However, in a continuous treatment regime, e.g., dosage or duration of treatment, there is no notion of turning the
treatment "on/off".
%
Instead, we focus on two different notions of treatment effects as a proxy for
the effectiveness of the prescribed treatment.

First, we look at the average effect of a slight increase in the treatment/dosage of the population, which we call
Average Treatment Derivative (ATD) and define it as the following:
%
\begin{definition}[Average Treatment Derivative]
For the treatment regime $f_T$ in SCM $\scm$, we define the average treatment derivative (ATD) as 
\begin{align}
    \text{ATD}_{\scm} = \E_{\vect{u} \sim P_{\vect{U}}}\left[\frac{\partial Y_{t}(\vect{u})}{\partial t}\Big|_{t=T(u)}\right],
    \label{eq:atd}
\end{align}
%where
%\begin{align}
%    \frac{\partial Y_{T(\vect{u})}(\vect{u})}{\partial T(\vect{u})}
%    := \lim_{\epsilon \todown 0}
%        \frac{ Y_{T(\vect{u}) + \epsilon}(\vect{u}) - Y_{T(\vect{u}) - \epsilon}(\vect{u})}{2\epsilon}
%\end{align}
\end{definition}

Next, we consider the continuous version of ATE by comparing the average causal effect of an arbitrary treatment/dosage
to the average causal effect at $T=0$.
%
We call this quantity Average Dose Effect (ADE):
\begin{definition}[Average Dose Effect]
    The average dosage effect (ADE) of the treatment at $T=d$ for SCM $\scm$ is defined as
    \begin{align}
        \text{ADE}_{\scm}(d) := \E_{\vect{u}\sim P_{\vect{U}}}[Y_{\scm(T=d)}(\vect{u}) - Y_{\scm(T=0)}(\vect{u})]
        \label{eq:ade}
    \end{align}
\end{definition}
Note that we cannot readily use eq.~\ref{eq:atd}/eq.~\ref{eq:ade} to estimate the ATD/ADE, as we only have access to the observational
distribution $P$ and the causal graph $\graph$ and not the latent distribution $P_\vect{U}$.
%
In fact, ATD/ADE are generally non-identifiable, i.e., there exist multiple SCMs with the same causal graph $\graph$ and
generated distribution $P$ that result in different values of ATD/ADE.
%
For some graphs, however, one can use identification algorithms like $do$-calculus to identify the causal effect from the
observational distribution~\citep{causal-pearl}.
%
Even in identifiable cases, because of noisy measurements and finite number of samples, the value of ATD/ADE cannot be
point-identified \vahid{1-Give some examples both in the experiments and by citing papers. Give some examples here or
in the Appendix for the (non-)identifiability of ATD and relate it to the identifiability of Pearl's do-interventions}.
%
\subsection{Partial identification of ATD/ADE}
Though it is not possible to point-identify the value of ATD/ADE for general SCMs, we may still be interested in partially identifying
them, i.e., finding the tightest bound over their values.
%
In literature, the partial identification problem is defined for ATEs~\citep{manski2003partial}.
%
Here we extend the definition to ATD and ADE:
\begin{definition}[Partial Identification of ATD/ADE]
    \label{def:partial-id}
    Partial identification of ATD is the solution to the following optimization problem:
    \begin{align}
        & (\min_{{\scm'} \in \mathfrak{M}} \text{ATD}_{\scm'},\;
        \max_{{\scm'} \in \mathfrak{M}} \text{ATD}_{\scm'}) \nonumber \\[3pt]
        &\text{ s.t.}\ P_{\scm'} = P\nonumber \\
        &\text{\space~\space~\space~\space}\ \graph_{\scm'} = \graph
        \label{opt:PI}
    \end{align}
    where $\mathfrak{M}$ is the set of all SCMs on random variables $\vect{V}$.
    %
    We denote the solution to above optimization problem with $(\lowerATD, \upperATD)$.
    %
    Similarly, we can define the partial identification of ADE by replacing $\text{ATD}_{\scm'}$ with $\text{ADE}_{\scm'}(d)$
    in eq.~\ref{opt:PI}.
    %
    We call the solution to the latter optimization problem as $(\lowerADE(d), \upperADE(d))$.
\end{definition}
%
%\vahid{Discuss the following with @Rahul:} one may claim that the notion of ATD is not a good proxy for estimating
%effectiveness of a treatment regime.
%%
%For example, consider the following average response curve of treatment dosage on the outcome:
%\begin{figure}[H]
%\centering
%    \begin{tikzpicture}
%        \draw[->] (-3,0) -- (3,0) node[right] {$T$};
%        \draw[->] (0,0) -- (0,3) node[above] {$Y_T$};
%
%        \draw[thick,purple,domain=-2.5:2.5,smooth] plot (\x,{0.5*(\x)^2});
%    \end{tikzpicture}
%\caption{The response curve $Y_T$ for a treatment regime.} \label{fig:example-atd}
%\end{figure}
%The ATD for the above response curve is 0.
%%
%However, for treatments $T \geq 0$, the effect is positive and our objective does not capture that.
%%
%In fact, one may be interested in comparing the effect of two dosage values $T=l$ and $T=h$:
%\begin{align}
%    \E[Y_{h}] - \E[Y_{l}]
%\end{align}
%We claim that bounding the value of ATD naturally results in a bound over quantities like $\E[Y_{h}] - \E[Y_{l}]$:
%%
%\begin{align}
%    \E[Y_{h}] - \E[Y_{l}]
%    &= \E_{\vect{u}\sim P_{\vect{U}}}[Y_{T=h}(\vect{u}) - Y_{T=l}(\vect{u})] \nonumber \\
%    &= \E_{\vect{u}\sim P_{\vect{U}}}[\int_{l}^h \frac{\partial Y_{T=t}(\vect{u})}{\partial t} dt] \nonumber \\
%    &= \int_{l}^h \E_{\vect{u}\sim P_{\vect{U}}} [\frac{\partial Y_{T=t}(\vect{u})}{\partial t}] dt
%\end{align}
%
%Now, if we show that maximizing/minimizing $\E\left[\frac{\partial Y_{T(\vect{u})}(\vect{u})}{\partial T(\vect{u})}\right]$
%results in maximizing/minimizing $\E\left[\frac{\partial Y_{T=t}(\vect{u})}{\partial t}\right]$ for every $t \in [l, h]$,
%we reach a bound over $\E[Y_{h}] - \E[Y_{l}]$. \vahid{I think this can be proved by the positivity assumption.
%We should talk with Vasilis.}

==> figures/experiments.tex <==
We start by showing the performance of our algorithm in simple synthetic settings for both identifiable and non-identifiable causal graphs with discrete and continuous endogenous variables. 
\subsection{Identifiable Targets}
\xhdr{Frontdoor Graph} For our first experiment, we consider the Frontdoor causal graph (Figure \ref{fig:frontdoor-graph}) with binary $X, Y, W \in \{0, 1\}$. We use the same SCM as in \citet{parital-ident-elias}:
\begin{align}
    U_1 &\sim \text{Unif}(0, 1) \nonumber \\
    U_2 &\sim \text{Normal}(0, 1) \nonumber \\
    X &\sim \text{Binomial}(1, U_1)\nonumber \\
    W &\sim \text{Binomial}(1, \frac{1}{1 + exp(-X-U_2)}) \nonumber\\
    Y &\sim \text{Binomial}(1, \frac{1}{1+exp(W -U_1)})
\end{align}
We are interested in estimating $\E[Y_{(X=0)}]$. Figure \ref{fig:frontdoor-estimate} shows that our result on $N=10^4$ samples matches the actual ACE = $0.5085$. \vahid{In \citet{parital-ident-elias}, they construct credible intervals over the value of interest}

\xhdr{Backdoor Graph} Next, we evaluate our algorithm on a continuous SCM with backdoor causal graph (Figure \ref{fig:backdoor-graph}). We consider a linear Gaussian SCM, where
\begin{align}
    X &\sim \text{Normal}(0, 1) \nonumber\\
    T &\sim \text{Normal}(X, 2) \nonumber\\
    Y &\sim \text{Normal}(T+X, 1)
\end{align}
\begin{figure}
    \centering
    \includegraphics[scale=0.7]{figures/backdoor-lower.png}
    \caption{Lower bound response function and generated data for the Backdoor graph}
    \label{fig:backdoor-response}
\end{figure}
The true value of ACE is $\E[Y_{T=0}] = 0$. Figure \ref{fig:backdoor-response} shows the average response functions $\E[Y_{T=t}]$ corresponding to the upper/lower bounds of $\E[Y_{T=0}]$. Though the actual value of ACE is identifiable, we still observe a gap between upper/lower bounds due to the non-zero Sinkhorn divergence between the true observational distribution and the generated distribution. We have the following observations:
\begin{itemize}
    \item The gap converges to a finite number as shown in figure \ref{fig:backdoor-convergence}. Otherwise, the Sinkhorn divergence will not go to zero.
    \item One can argue that the response function in \ref{fig:backdoor-response} is the true response function that generates a similar distribution to the observed one. However, if we limit the data to the neighborhood of $T=0$, we observe the Sinkhorn divergence is much larger. To address this issue, we can consider a new cost function that puts more weights on the points in the neighborhood $(t-\delta, t+\delta)$. For example, in a 2d SCM with variables $(T, Y)$, we can define the new cost function as
    \begin{align}
        C_\lambda((t', y'), (t'', y'')) := \begin{cases}
        ||t'-t''|| + \lambda ||y'-y''|| & \text{ if } t', t''\in (t-\delta, t+\delta) \\
        ||t'-t''|| +  ||y'-y''|| & \text{ o.w.}
        \end{cases}
    \end{align}
    for some $\lambda > 1$.
    
    \item One can also limit the form of the response function by assuming Lipschitz constraints on the whole function or the neighborhood $(t-\delta, t+\delta)$. Figure \ref{fig:backdoor-lipschitz} demonstrates this idea. Also, one can stick to simple function forms like polynomials, linear combinations of non-linear basis functions, etc (\citet{iv-continuous}).
\end{itemize}

\subsection{Non-identifiable Targets}
\xhdr{Bow Graph (Discrete)} We consider the Bow causal graph (Figure \ref{fig:bow-graph}) with binary $X, Y \in \{0, 1\}$. The goal is to estimate the probability of necessity and sufficiency (PNS) $P(Y_{X=1}=1, Y_{X=0}=0) = \E[Y_{X=1} (1-Y_{X=0})]$. We consider the SCM in \citet{parital-ident-elias}:
\begin{align}
        U &\sim \text{Normal}(0, 1) \nonumber \\
    X &\sim \text{Binomial}(1, \frac{1}{1+exp(U)})\nonumber \\
    E &\sim \text{Logistic}(0, 1) \nonumber\\
    Y & \gets \II(X-U+E+0.1 > 0)
\end{align}
It can be shown that the optimal bound on PNS is $(0, 0.6775)$. Figure \ref{fig:bow-estimate} shows the result of our algorithm by running on $N=10^3$ samples.

\xhdr{Bow Graph (Continuous)} Consider the following linear Gaussian SCM for two continuous endogenous variables $T, Y$:
\begin{align}
    U &\sim \text{Normal}(0, 1) \nonumber \\
    T &\sim \text{Normal}(U, 1) \nonumber \\
    Y &\sim \text{Normal}(T+U, 1)
\end{align}
The value of $\E[Y_{(T=1)}] - \E[Y_{(T=0)}]$ is non-identifiable from the observational distribution (\vahid{In fact, we can show there is no informative bound over it}). Figure \ref{fig:bow-response} shows the average response functions $\E[Y_{(T=t)}]$ corresponding to the upper/lower bound of $\E[Y_{(T=1)}] - \E[Y_{(T=0)}]$ by constraining them to 5-Lipschitz functions (Otherwise, the gap between upper bound and lower bound will go to infinity).

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/bow_response.png}
    \caption{Upper/lower bound response functions and generated data for the Bow graph.}
    \label{fig:bow-response}
\end{figure}
  
